PingAn-VCGroup's Solution for ICDAR 2021 Competition on Scientific Literature Parsing Task B: Table Recognition to HTML

This paper presents our solution for ICDAR 2021 competition on scientific literature parsing taskB: table recognition to HTML. In our method, we divide the table content recognition task into foursub-tasks: table structure recognition, text line detection, text line recognition, and box assignment.Our table structure recognition algorithm is customized based on MASTER [1], a robust image textrecognition algorithm. PSENet [2] is used to detect each text line in the table image. For text linerecognition, our model is also built on MASTER. Finally, in the box assignment phase, we associatedthe text boxes detected by PSENet with the structure item reconstructed by table structure prediction,and fill the recognized content of the text line into the corresponding item. Our proposed methodachieves a 96.84% TEDS score on 9,115 validation samples in the development phase, and a 96.32%TEDS score on 9,064 samples in the final evaluation phase.

==> tmp.tex <==


\author{
 Jiaquan Ye \\
  Visual Computing Group,\\
  Ping An Property & Casualty Insurance Company\\
  \texttt{jiaquanye@qq.com} \\
  %% examples of more authors
   \And
 Xianbiao Qi \\
  Visual Computing Group,\\
  Ping An Property & Casualty Insurance Company\\
  \texttt{qixianbiao@gmail.com} \\
  \And
 Yelin He \\
  Visual Computing Group,\\
  Ping An Property & Casualty Insurance Company\\
  \texttt{xxxx@qq.com} \\
  %% \AND
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
  %% \And
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
  %% \And
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
}



\author{
 Jiaquan Ye, \And Xianbiao Qi\thanks{1}, \And Yelin He, \And Yihao Chen, \And Dengyi Gu, \And Peng Gao, \And Rong Xiao \\
 \newline
 1. Visual Computing Group,\\
  Ping An Property \& Casualty Insurance Company.\\
 2. Ping An Tech Company.\\
  \texttt{jiaquanye@qq.com, qixianbiao@gmail.com}
}




\author{
 Jiaquan Ye, \And Xianbiao Qi\thanks{1}, \And Yelin He, \And Yihao Chen, \And Dengyi Gu, \And Peng Gao, \And Rong Xiao \\
 \newline
 1. Visual Computing Group,\\
  Ping An Property \& Casualty Insurance Company.\\
 2. Ping An Tech Company.\\
  \texttt{jiaquanye@qq.com, qixianbiao@gmail.com}
}





\author{
 Jiaquan Ye \And Xianbiao Qi \\
 \newline
 
 \And Yelin He \And Yihao Chen \And Dengyi Gu \And Peng Gao \And Rong Xiao \\
 
 
 Visual Computing Group,\\
  Ping An Property \& Casualty Insurance Company\\
  \texttt{jiaquanye@qq.com, qixianbiao@gmail.com} \\

}




\author[1]{AAAAA}
\author[1]{Bob Jones}\\
\author[2]{sssss}

\author[1]{BDDDb Jones}\\

\affil[1]{Department of Mathematics, University X}
\affil[2]{Department of Biology, University Y}
\newline








\begin{table*}
\begin{floatrow}
\centering
\capbtabbox{
 \begin{tabular}{l|c}
\hline
\textbf{Optimizer}                & \multicolumn{1}{l}{\textbf{Sturcture Word Acc}} \\ \hline
Adam & 0.7784                                            \\ \hline
Ranger         & \textbf{0.7826}                                            \\ \hline
\end{tabular}
}{
 \caption{(a)}
 \label{tab:tb1}
}
\capbtabbox{
 \begin{tabular}{c|c}
\hline
\textbf{Feature Fusion}            & \textbf{Content Word Acc} \\ \hline
No & 0.9313                               \\ \hline
Yes        & \textbf{0.9347}                               \\ \hline
\end{tabular}
}{
 \caption{(b)}
 \label{tab:tb2}
}
\end{floatrow}
\end{table*}







\begin{table}[h]
\centering
\begin{tabular}{ccc|c}
\hline
\textbf{ESB} & \textbf{SyncBN} & \textbf{CL} & \textbf{Structure Token Acc.} \\ \hline
\checkmark            &                 &             & 0.7734                        \\ \hline
\checkmark            & \checkmark               &             & 0.7750                        \\ \hline
\checkmark            & \checkmark               & \checkmark           & \textbf{0.7785}                        \\ \hline
\end{tabular}
\caption{Ablation studies of ESB, SyncBN and CL on development phase validation dataset. ESB:empty space box encoding, encode \emph{<td></td>} and \emph{<td> </td>} separately; SyncBN:Synchronized BatchNorm for multi-GPU training; CL:concatenate output of transformer layers.}
\end{table}

